Forward Invariant Cuts to Simplify Proofs of Safety

The use of deductive techniques, such as theorem provers, has several advantages in safety verification of hybrid sys- tems; however, state-of-the-art theorem provers require ex- tensive manual intervention. Furthermore, there is often a gap between the type of assistance that a theorem prover requires to make progress on a proof task and the assis- tance that a system designer is able to provide. This paper presents an extension to KeYmaera, a deductive verification tool for differential dynamic logic; the new technique allows local reasoning using system designer intuition about per- formance within particular modes as part of a proof task. Our approach allows the theorem prover to leverage for- ward invariants, discovered using numerical techniques, as part of a proof of safety. We introduce a new inference rule into the proof calculus of KeYmaera, the forward invariant cut rule, and we present a methodology to discover useful forward invariants, which are then used with the new cut rule to complete verification tasks. We demonstrate how our new approach can be used to complete verification tasks that lie out of the reach of existing deductive approaches us- ing several examples, including one involving an automotive powertrain control system.

==> generic.macros.tex <==
% Generic
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% English
\newcommand{\ie}{{i.e.}\xspace}
\newcommand{\Ie}{{I.e.}\xspace}
\newcommand{\eg}{{e.g.}\xspace}
\renewcommand{\etc}{{etc.}\xspace}
\newcommand{\viz}{{viz.\xspace}}
\newcommand{\etal}{{et al.}\xspace}

% Generic refs
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{tab:#1}}

\newcommand{\matlab}{MATLAB}
\newcommand{\mathematica}{Mathematica}

% Comments, Reviewing, Formatting
\newcommand{\ignore}[1]{}

% General Math
\newcommand{\setof}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\sublist}[2]{\ensuremath{#1_{1},\ldots,#1_{#2}}}
\newcommand{\suplist}[2]{\ensuremath{#1^{1},\ldots,#1^{#2}}}


% Complexity
\newcommand{\npcomplete}{\textsc{Np}-\textsc{complete}\xspace}
\newcommand{\nphard}{\textsc{Np}-\textsc{Hard}\xspace}
\newcommand{\nlogspace}{\textsc{NLogspace}\xspace}
\newcommand{\pspace}{\textsc{PSpace}\xspace}
\newcommand{\expspace}{\textsc{ExpSpace}\xspace}

\newcommand{\mcl}[1]{\multicolumn{1}{l}{#1}}
\newcommand{\mcc}[1]{\multicolumn{1}{c}{#1}}

\newcommand{\mypara}[1]{\vspace{0.5em}\noindent{\bf #1.}}
\newcommand{\myipara}[1]{\vspace{0.5em}\noindent{\em #1.}}

% math
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Integers}{\mathbb{Z}}
\newcommand{\Rationals}{\mathbb{Q}}


==> ha_ecs.tex <==
\begin{figure}[t!]
\centering
\begin{tikzpicture}[>=stealth']
\tikzstyle{smalltext}=[font=\fontsize{7}{7}\selectfont]
\tikzstyle{state}=[smalltext,rectangle,rounded corners,draw,minimum height=2em,inner sep=2pt,align=center]

\node[state] (startup) {$\begin{array}{l}
                        \textbf{startup} \\
                        \dot{\vx} = f_{startup}(\vx)
                        \end{array}$};
\node[state,node distance=50mm,right of=startup] (normal) {%
                        $\begin{array}{l}
                        \textbf{normal} \\
                        \dot{\vx} = f_{normal}(\vx)
                        \end{array}$};
\node[coordinate,node distance=40mm,left of=startup] (init) {};

\draw[->] (startup) to node[above,smalltext] {$\tau \ge 8ms$} (normal);
\draw[->] (init) to node[near start,above,smalltext]
{$\begin{array}{l} |p| \le 0.001, |r| \le 0.001, \\
                   i = 0, t = 0
  \end{array}$} (startup); 

\end{tikzpicture}
\caption{Hybrid Automaton for Engine Fuel Control System\label{fig:ha_ecs}}
\end{figure}



==> proofoflemma.tex <==
\subsection{Proof of \rref{lemma:iorelation_containment} }
We prove by structural induction on $\alpha$. 
\begin{enumerate}
\item For the case $\alpha = (x:=a)$, we have 
$\rho_{I,\eta}(\alpha \downarrow D) =  \rho_{I,\eta}((x := a) \downarrow D) = \rho_{I,\eta}(?D; x:=a; ?D)$,
which is $\rho_{I,\eta}(?D) \circ \rho_{I,\eta}(x := a) \circ \rho_{I,\eta}(?D)$, which 
is equivalent to $\rho_{I,\eta}(\alpha) \cap (\mathbf{D} \times \mathbf{D})$, and the lemma follows.
\item This case is analogous to the previous case. 
\item By equational reasoning,
\begin{align}
\rho_{I,\eta}(?\phi \downarrow D) &= \rho_{I,\eta}(?(\phi~\wedge~D)) \\
&= \{(\nu, \nu) | val_{I, \eta}(\nu, \phi~\wedge~D) = {\tt true} \}\\
&= \{(\nu, \nu) | val_{I, \eta}(\nu, \phi) ~\wedge~val_{I, \eta}(\nu, \phi) = {\tt true} \}\\
&= \rho_{I,\eta}(?\phi) \cap (\mathbf{D}\times\mathbf{D})
\end{align}
\item Suppose $(\nu, \omega) \in \rho_{I,\eta}(\{x_1' = \theta_1, \dots, x_n' = \theta_n \&~H \} \downarrow D)$. Then for some $r \ge 0$, there
is a function $f:[0,r] \mapsto \text{Sta}(\Sigma)$ such that $f(0) = \nu$, $f(r) = \omega$ that respects
the differential equations (as described in \cite{PlatzerThesis}) 
and respects $val_{I,\eta}(f(\zeta), \xi) = {\tt true}$ for each $\zeta \in [0,r]$ and each state
$\xi \in \textgoth{m}(H~\wedge~D)$. It follows that $\nu, \omega \in \mathbf{D}$, and the
required inclusion follows.
\item As an induction hypothesis, suppose the lemma holds for hybrid programs $\beta$, $\gamma$, and consider $\alpha = (\beta; \gamma)$
\begin{align}
\rho_{I,\eta}((\beta; \gamma) \downarrow D) &= \rho_{I,\eta}( (\beta \downarrow D); (\gamma \downarrow D) )\\
&= \rho_{I,\eta}(\beta \downarrow D) \circ \rho_{I,\eta}(\gamma \downarrow D)\\
&\subseteq (\rho_{I,\eta}(\beta) \cap( \mathbf{D} \times \mathbf{D} )) \circ (\rho_{I,\eta}(\gamma \downarrow D) \cap (\mathbf{D} \times \mathbf{D})\\
&\subseteq(\rho_{I,\eta}(\beta)\circ \rho_{I,\eta}(\gamma))\cap (\mathbf{D} \times \mathbf{D}) \\
&\subseteq\rho_{I,\eta}(\beta; \gamma) \cap (\mathbf{D} \times \mathbf{D})
\end{align}
\item As an induction hypothesis, suppose the lemma holds for hybrid programs $\beta$, $\gamma$, and consider $\alpha = (\beta \cup \gamma)$
\begin{align}
\rho_{I,\eta}((\beta; \gamma) \downarrow D) &=\rho_{I,\eta}( (\beta \downarrow D) \cup (\gamma \downarrow D) )\\
&\subseteq \rho_{I,\eta}( (\beta \downarrow D) ) \cup \rho_{I,\eta}(\gamma \downarrow D)\\
&\subseteq (\rho_{I,\eta}( \beta ) \cap (\mathbf{D} \times \mathbf{D})) \cup (\rho_{I,\eta}(\gamma \downarrow D) \cap (\mathbf{D} \times \mathbf{D}))\\
&\subseteq (\rho_{I,\eta}(\beta \cup \gamma) \cap (\mathbf{D} \times \mathbf{D}))
\end{align}
\item As an induction hypothesis, suppose the lemma holds for the hybrid program $\beta$, and consider $\alpha = (\beta)^*$.
\begin{align}
\rho_{I,\eta}(\beta^* \downarrow D) &= \rho_{I,\eta}(?D) \circ \bigcup_{i \in \mathbb{N}} \rho_{I,\eta}(\beta \downarrow D)^i\\
& \subseteq \rho_{I,\eta}(?D) \circ \bigcup_{i \in \mathbb{N}} (\rho_{I,\eta}(\beta) \cap (\mathbf{D} \times \mathbf{D}))\\
& \subseteq \left(\bigcup_{i \in \mathbb{N}} \rho_{I,\eta}(\beta)^i\right) \cap (\mathbf{D} \times \mathbf{D})\\
& \subseteq \rho_{I,\eta}(\beta^*) \cap (\mathbf{D} \times \mathbf{D})
\end{align}
\end{enumerate}
\qed


==> toolsupport.tex <==
We describe the partial automation for our approach based on a \matlab implementation. 
The implementation requires the designer to enter a description of the dynamics (in the form of ODEs) 
for each mode believed to contain useful forward invariants, based on designer intuition.
Numerical techniques are then used to synthesize forward invariant candidates. The soundness of the candidates are then checked using the dReal tool.
The implementation leverages several numerical technique to find the forward 
invariants.

%with the tool Manticore, which we
%plan to release at a future date.
%Manticore accepts a hybrid program specification of a system, along with user
%annotations about regions that are believed to contain forward invariants.
%Manticore first checks to see if the annotations themselves are invariants of
%the continuous system, and if this is the case, generates a partial proof file
%with the annotations as forward invariant cuts.
%Otherwise, Manticore examines the differential equations that appear in the
%hybrid program and attempts to synthesize a forward invariant. Manticore
%leverages several techniques to find forward invariants.

\begin{enumerate}
\item If the system dynamics are linear and stable, a Lyapunov function can be
readily computed by solving the Lyapunov equation (\ref{eq:lyaplinear}) for the autonomous components.
%If the dynamics are linear but not stable, a theorem due to Taussky \cite{}
%allows us to compute a barrier function for the autonomous dynamics by solving a
%Sylvester equation.

\item If the system is polynomial, our implementation attempts to compute a
sum-of-squares Lyapunov function following the development of \cite{Prajna2005}.

\item If all of the above fail, our implementation uses the simulation-driven approach
described in \cite{Kapinski14} to search for a barrier certificate, as described in 
Sec. \ref{sec:safeinvs}.
\end{enumerate}

Once a forward invariant has been computed, 
a partial proof file for \keymaera is generated 
that uses the forward invariant to apply the forward
invariant cut rule.
This partial proof file can then be loaded in \keymaera to finish the proof task.

%\begin{figure}
%\label{fig:manticoreoverview}
%\centering
%includgraphics[width=\textwidth]{img/manticoreoverview}
%\caption{The tool Manticore takes as input a hybrid program representation of a
%system, computes forward invariants using several heuristics, and uses the
%forward invariant cut rule to simplify the proof task. The result is a partial
%proof file, which can then be sent to KeYmaera to finish proving.}
%\end{figure}






